Cost-aware Integration Process Modeling in Multiclouds

Integration as a service (INTaaS) is the centrepiece of current corporate, cloud and device integration processes. Thereby, compositions of integration patterns denote the required integration logic as integration processes, currently running in single-clouds. While multicloud settings gain importance, their promised freedom of selecting the best option for a specific problem is currently not realized as well as security constraints are handled in a cost-intensive manner for the INTaaS vendors, leading to security vs. costs goal conflicts, and intransparent to the process modeler. In this work, we propose a design-time placement for processes in multiclouds that is cost-optimal for INTaaS problem sizes, and respects configurable security constraints of their customers. To make the solution tractable for larger, productive INTaaS processes, it is relaxed by using a local search heuristic, and complemented by correctness-preserving model decomposition. This allows for a novel perspective on cost-aware process modeling from a process modeler's perspective. The multicloud process placement is evaluated on real-world integration processes with respect to cost- and runtime-efficiency, and discusses interesting trade-offs. The process modeler's perspective is investigated based on a new cost-aware modeling process, featuring the interaction between the user and the INTaaS vendor through ad-hoc multicloud cost calculation and correctness-preserving, process cost reduction proposals.

==> correctness.tex <==
\labeltitle{Cutting} Similar to \enquote{component decomposition} in Silva et al. \cite{DBLP:conf/europar/SilvaP17}, we study pre-partitioning of compositions into smaller shareable and non-shareable sub-compositions (cf. (a)). This increases the number of compositions, but leads to smaller compositions that might be placed more efficiently ($\rightarrow$ hypothesis \emph{HB}).

Algorithmically, we use the side-effect free and \emph{correcntess-preserving} graph re-writing approach from~\cite{DBLP:conf/debs/0001MFR18}, which is based on double-pushouts from Category Theory, and thus allows for a visual definition of a re-write rule.
Thereby, the correctness is guaranteed on a composition level, if the contracts of neighbor patterns match according to~\cref{def:ipcg}.
In our case, we are interested in connected sub-compositions that are non-shareable.
%\begin{wrapfigure}{l}{0.5\linewidth}
%	%%%\vspace{-0.5cm}
%	\centering
%	\includegraphics[width=0.55\columnwidth]{images/nonshareable_patterns}
%	%%\vspace{-0.5cm}
%	\caption{Non-shareable sub-graph rewriting}
%	\label{fig:nonshareable_rewriting}
%	%%\vspace{-0.6cm}
%\end{wrapfigure}
These parts are cut from the original composition, replaced by a request-reply pattern (denoted by sender adapter S and receiver adapter R), and then moved to another composition with an inverse pair of receiver and sender adapters to guarantee its functional correctness (but adding latency through the remote call).

%\begin{figure}[bt]
%	\centering
%	\includegraphics[width=0.5\columnwidth]{images/nonshareable_patterns}
%	\caption{Non-shareable sub-graph rewriting}
%	\label{fig:nonshareable_rewriting}
%\end{figure}

This is formally specified in~\cref{fig:nonshareable_rewriting} and used to evaluate hypothesis HB further in subsequent case studies.
The rewriting in~\cref{fig:nonshareable_rewriting} moves non-shareable sub-compositions $SSQ_1$ into an extra composition, that requires an inbound message receiving pattern $P_4$ and sends the resulting message via a new sender $P5$ pattern.
From the perspective of the original composition (\ie $P_1$ to $P_2$), a Request-Reply pattern with a sender $P_3$ and message receiving pattern $P_6$ is added.

\begin{lemma}
	The rewriting in~\cref{fig:nonshareable_rewriting} results to correct pattern compositions according to matching contracts in~\cref{def:ipcg}.
\end{lemma}

\begin{proof}[Proof (sketch)]
	The rewriting in~\cref{fig:nonshareable_rewriting} is correct, if the pattern contracts match, \ie conditions $Cx$ hold:
	\begin{itemize}
		\item[C1] the request pattern pair $P_3$ to $P_4$ specifies its data elements $EL$ corresponding to the original $P_1$ to $SSQ'_1$, and $P_5$ to $P_6$ same as $SSQ'_1$ to $P_2$,
		\item[C2] and the contract properties $CPT$ are compatible.
	\end{itemize}
	Condition C1 holds by definition of~\cref{fig:nonshareable_rewriting}.
	For C2 we need to look into the specification of the $CPT$ of send and receive patterns from~\cite{DBLP:conf/debs/0001MFR18}.
	With $CPT_{send}= \{(ENC,no), (ENCR,no), (SIGN,no)\} =CPT_(receive)$ for $inContr$ and $outContr$, C2 is correct as well.
\end{proof}

Note that for message level security enabled, we would have $CPT_{send}= \{(ENC,no), (ENCR,true), (SIGN,no)\} =CPT_{receive}$, for $inContr$ and $outContr$, which is still correct, however, practically requires an additional Encryptor and Decryptor patterns on the left-hand side between $P_1$ to $SSQ_1$, $SSQ_1$ to $P_2$, respectively.
Then this needs to be reflected on the right-hand side with Encryptor patterns between $P_1$ and $P_3$ as well as $SSQ'_1$ and $P_5$, and Decryptor patterns between $P_4$ and $SSQ'_1$ as well as $P_6$ and $P_2$.
With $CPT_{encrypt}=$ $\{(ENC,any), (ENCR,no), (SIGN,any)\}$ for $inContr$ and $CPT_{encrypt}= \{(ENC,any), (ENCR,yes), (SIGN,any)\}$ for $outContr$, the respective contracts of the patterns' neighbours are matched.
This is the same for the Decryptor with $CPT_{decrypt}= \{(ENC,any),\\ (ENCR,yes), (SIGN,any)\}$ for its $inContr$ and $CPT_{decrypt}=\\ \{(ENC,any), (ENCR,no), (SIGN,any)\}$ for its $outContr$. 





\subsection{Process change correctness}
\label{sub:op:correctness}
%
    don't discuss encryption etc in detail since pattern contracts were not introduced properly.
    instead give an example later in the proof.
    boundaries were also not introduced! hence no bisimulation argument.

We now show that the optimizations do not change the input-output behaviour of the pattern graphs in the timed db-nets semantics, \ie if we have a rewrite rule from graph $G$ to graph $G'$ as $G \Rightarrow_{r,g} G'$ (cf.~\cref{def:op:rule_application} (on~\cpageref{def:op:rule_application})), then the constructed \tdbnet with boundaries $\sem{G}$ has the same observable behaviour as that of $\sem{G'}$ (cf.~\cref{sec:interpretation-atomic}).
More formally, having the \enquote{same input-output behavior} requires that the transition systems of the original and the rewritten graphs are bisimilar in a certain sense (cf. \tdbnet transition system based on \dbnet in~\cref{sub:pn:db-net,sub:pc:tdbn_boundaries}), as more formally defined in~\cref{def:op:bisimilarity}.
For being bisimilar, it is required that the left hand side of a rewrite can simulate the right hand side, and vice versa.
\todo[inline]{inline timed dbnets execution semantics}
\begin{definition}[Bisimulation] 
	\label{def:op:bisimilarity}
    Let $\Gamma^\mathcal{B}_{s_0} = \langle S, s_0, \rightarrow \rangle$ and $\Gamma^\mathcal{B'}_{s_0} = \langle S', s'_0, \rightarrow' \rangle$ be the associated labelled transition systems of two \tdbnets $B$ and $B'$ with the same boundaries from~\cref{sub:pn:db-net,sub:pc:tdbn_boundaries}, respectively.
    We say that a $B$-snapshot $(I, m)$ is functionally \emph{equivalent} to a $B'$-snapshot $(I', m')$, $(I, m) \approx (I', m')$,  if $I = I'$, and $m$ and $m'$ agree on output places, \ie for every output place $p$ with $m(p) = (\alpha, \gamma, age)$ and $m'(p) = (\alpha', \gamma', age')$, we have $\alpha = \alpha'$, for the elements that are in the message $\alpha$, and those that are not required by any endpoint $\gamma$ (usually $\gamma = \emptyset$), and $age$ is the timed db-net age information. 
    % $\bullet$ denotes the required fields of a message, $\alpha$ the fields that are in the message, but not required by any endpoint, $\gamma$ is the header information about the origin of a message (\eg sender), and $age$ is the timed db-net age information.
    % \TODO{need to restrict $B$ and $B'$ so this makes sense}
    % \TODO{compare the headers?}
    
    Further we say that $\Gamma^\mathcal{B}_{s_0}$ is functionally \emph{equivalent} to $\Gamma^\mathcal{B'}_{s_0}$, $\Gamma^\mathcal{B}_{s_0} \sim \Gamma^\mathcal{B'}_{s_0}$, if whenever $s_0 \rightarrow^* (I, m)$ then there is $(I', m')$ such that $s'_0 \rightarrow'^* (I', m')$ and $(I, m) \approx (I', m')$ and $\Gamma^\mathcal{B}_{(I,m)} \sim \Gamma^\mathcal{B'}_{(I',m')}$, and whenever $s'_0 \rightarrow^* (I', m')$ then there is $(I, m)$ such that $s_0 \rightarrow^* (I, m)$ and $(I', m') \approx (I, m)$. \qedblack
%TODO    \todo[inline]{Probably need to tweak this definition; for instance, need $s_0$ to be all input places?}
\end{definition}
%Therefore we consider a bisimulation argument of the LTS of the timed db-net of the rewrite rule's LHS, and the LTS of the timed db-net of its RHS.
Note that this bisimulation definition neglects the unused fields $\gamma$ as well as the age of the tokens $age$, since $\gamma$ is used for deciding on the efficiency of a data reducing optimization only and the age information is anyway reset when moved to a new place (cf.~\cref{sub:pn:timed_db_nets}).
Let us discuss an explanatory example of bisimulation. 

\begin{example}
	\Cref{fig:op:bisimilarity_example} shows the interpretation of a simple IPCG as a \tdbnet before and after applying the rewrite rule for the combining sibling patterns from~\cref{fig:combine_sibling_nodes_v2_b} (for simplicity without boundaries).
	\begin{figure}[bt]
		\begin{center}$
			\begin{array}{c}
			\subfigure[Before applying the rewrite rule]{\label{fig:op:bisimilarity_example_1}\includegraphics[width=1\columnwidth]{images/tdbnet_combine_sibling_left}} \\
			\subfigure[After applying the rewrite rule]{\label{fig:op:bisimilarity_example_2}\includegraphics[width=1\columnwidth]{images/tdbnet_combine_sibling_right}}        
			\end{array}$
		\end{center}
		\caption{Timed db-net translation of IPCGs before and after applying the \enquote{combine sibling patterns} rewrite rule}
		\label{fig:op:bisimilarity_example}
	\end{figure}
	The improvement of the optimization is to move $SG_1$ (isomorphic to $SG_2$) in front of the forking pattern $F$ and leave out $SG_2$, which reduces the modeling complexity on the right hand side (cf.~\cref{fig:op:bisimilarity_example_2}).
	The synchronization subnet \emph{synch} is required to show bisimilarity between the original and the resulting net, since tokens might be moved independently in $SG_1$ and $SG_2$ before applying the optimisation.
	The subnet (essentially transitions $T_{s1},T_{s2}$) compensates for that to ensure that places $P_2$ and $P_3$ can be reached independently as well.
	Hence according to \cref{def:op:bisimilarity}, the \tdbnet $B$ representing \cref{fig:op:bisimilarity_example_1} and $B'$ \cref{fig:op:bisimilarity_example_2} are bisimilar $\Gamma^\mathcal{B}_{(I,m)} \sim \Gamma^\mathcal{B'}_{(I,m')}$ for any database instance $I$, and any markings $m$ and $m'$ with $m(P_1) = m'(P_1)$ and $m(p) = \{\emptyset\}$,  $m'(p) = \{\emptyset\}$ for all other $p$. \qedblack
\end{example}
	% for $(I=\emptyset, m=(e_1,e_2))$ and $(I'=\emptyset, m'=(e_1,e_2))$.
% However, they are not bisimilar for $(I=\emptyset, m=(e_1,e_2))$ and $(I'=\emptyset, m'=(e_1))$. \qedblack

With the following congruence relation for the composition, we subsequently show the correctness of the optimizations by discussing the bisimilarity of the right and left hand sides of the respective optimization rules (first left to right, then right to left).

\begin{lemma}
    \label{thm:simulation-congruence}
    The relation $\sim$ is the congruence relation with respect to composition of timed db-nets with boundaries, \ie it is reflexive,
    symmetric and transitive.
    If $\Gamma^{\mathcal{B}_1}_{s_0} \sim \Gamma^{\mathcal{B}_1'}_{s_0}$, $\Gamma^{\mathcal{B}_2}_{s_0} \sim \Gamma^{\mathcal{B}_2'}_{s_0}$ for all $s_0$ on the shared boundary of $B_1$ and $B_2$, then $\Gamma^{\mathcal{B}_1 \circ \mathcal{B}_2}_{s_0} \sim \Gamma^{\mathcal{B}'_1 \circ \mathcal{B}'_2}_{s_0}$. \qedwhite
\end{lemma}

\begin{lemma}
	\label{thm:simulation-boundary}
	Let $G$ and $G'$ be IPCGs. 
	If $G \Rightarrow_{r,g} G'$ for an optimisation $r$, then $\sem{G}$ and $\sem{G'}$ have the same boundary.
\end{lemma}

\begin{theorem}[Optimization Correctness]
	With~\cref{thm:simulation-boundary}, let $s_0 = (I_0, m_0)$ be a snapshot for its \tdbnet with boundaries $\sem{G}$, and $s_0' = (I_0', m_0')$ a snapshot for $\sem{G'}$, such that $I_0 = I_0'$, and $m_0(p) = m_0'(p)$ for all places $p$ on the (shared) boundary of $\sem{G}$ and $\sem{G'}$, with $m_0$ and $m_0'$ otherwise empty. If $G \Rightarrow_{r,g} G'$ for some optimization $r$ and match $g$, then $\Gamma^{\sem{G}}_{s_0}$ is equivalent to $\Gamma^{\sem{G'}}_{s_0'}$.
\end{theorem}
%	Let $G$ and $G'$ be IPCGs.
%	If $G \Rightarrow_{r,g} G'$ for an optimisation $r$, then $\sem{G}$ and $\sem{G'}$ have the same boundary.
	% For every initial snapshot $s_0$ such that $s_0$ is a snapshot for both \tdbnets with boundaries $\sem{G}$ and $\sem{G'}$, if $G \Rightarrow_{r,g} G'$ for some rule $r$ and match $g$, then $\Gamma^{\sem{G}}_{s_0}$ is equivalent to $\Gamma^{\sem{G'}}_{s_0}$.

% Given an initial state $s_0$ for the transition system of the corresponding \tdbnet with boundaries $\Gamma^{\sem{G} _{s_0}}$ of each rewrite rule with tokens in boundary places.
% If $G \Rightarrow^* G'$, then $\Gamma^{\sem{G}}$ is equivalent to $\Gamma^{\sem{G'}}$.

\begin{proof}
	In each step, the rewriting modifies certain nodes.
	By~\cref{thm:simulation-congruence}, it is enough to show that the affected parts of the interpretation of the graphs are equivalent, which is done for each optimization subsequently.

\labelsubtitle{Redundant Sub-Processes}
Each move on the left hand side of the optimization rule in~\cref{fig:redundant_control_flow_v2} (on~\cpageref{fig:redundant_control_flow_v2}) either moves tokens into a cloud, out of a cloud, or inside a cloud.
In the first two cases, this can be simulated by the right hand side by moving the token through the CE or CBR and CF respectively followed by a move into or out of the cloud, while in the latter case the corresponding token can be moved in $SG'_1$ up to the isomorphism between $SG'_1$ and the cloud on the left.

Similarly, a move on the right hand side into or out of the cloud can easily be simulated on the left hand side. Suppose a transition fires in $SG'_1$. Since all guards in $SG'_1$ have been modified to require all messages to come from the same enriched context, the corresponding transition can either be fired in $SG_1$ or $SG_2$.
% \TODO{Right to left: only true if all patterns act on messages with the same context only.}

\todo[inline]{add cutting + proof; where to put the improvements?? move to section 2??}

% Focusing on minimal vendor costs (cf.~\cref{eq:minimal}) our model considers the introduced latencies only as an additional constraint and not as main objective.

% Our prototypical implementations uses GLPK\footnote{GNU Linear Programming Kit, visited 06/2020: \url{https://www.gnu.org/software/glpk/}} as MIP solver.

%TODO:\\
%- adding constraints: removal a lot of permutations of container variants: latency measurements\\
%- with sorting variants and without\\
%- show latency with pre-processing and without\\

%\subsection{Cost-efficient process placement}
%For Software-as-a-Service (SaaS) vendors (incl. INTaaS), the CEPP is a bin-packing problem, with a set of bins of different sizes and costs (\eg platforms or variants), and a set of items of different sizes (\eg pattern (sub-) compositions). 
%The objective is to find a cost efficient partitioning or assignment of the pattern compositions under the following constraints
%\begin{inparaenum}[\it C1] 
%	\item each IPCG is in exactly one container, \label{item:flowConstraint}
%	\item each container is exactly one variant, \label{item:containerConstraint}
%	\item the container size must not be exceeded by the assigned, required IPCG capacity, \label{item:sizeConstraint}
%	\item a no non-shareable IPCG is assigned to a container which contains compositions of a different tenant (security-awareness), \label{item:securityConstraint}
%	\item the maximum number of IPCGs per container is not exceeded, \label{item:maxFlowNumber}
%\end{inparaenum}
%which essentially means that the items can be incompatible to each other (\eg non-shareable), and thus cannot be in the same bin or incompatible to a bin (\eg logistic company not on competitor's platform AWS).
% since bin packing is NP-hard and the decision problem is NP-complete, we assume that this applies here as well.



==> timed_db_nets.tex <==
\subsubsection{Timed db-nets}
\label{sub:timed_dbnet}
%
We briefly recall the definition of \tdbnets \cite{DBLP:conf/edoc/0001RMRS18,ritter2019formal}, specifying the execution semantics of integration patterns.
A timed db-net is a Coloured Petri Net that has three layers: a persistence layer describing the underlying database of the net, a logic layer describing the queries
that can be made of the persistence layer, and a control layer
describing how tokens of data flow through the net, executing queries.
%
\begin{definition}[timed db-net~\cite{DBLP:conf/edoc/0001RMRS18,ritter2019formal}]
  \label{def:eip-net}
  A \emph{timed db-net} is a tuple $(\mathfrak{D},\mathcal{P},\mathcal{L},\mathcal{N}, \tau)$, where:
  \begin{compactitem}[$\bullet$]
    \item $\mathfrak{D}$ is a type domain --- a finite set of data types, each of the form $D = (\Delta_D, \Gamma_D)$, where $\Delta_D$ is a value domain, and $\Gamma_D$ is a finite set of domain-specific predicate symbols.
    \item $\mathcal{P}$ is a $\mathfrak{D}$-typed \textbf{persistence layer}, i.e., a pair $(\mathcal{R}, E)$, where $\mathcal{R}$ is a $\mathfrak{D}$-typed database schema, and $E$ is a finite set of first-order FO($\mathfrak{D}$) constraints over $\mathcal{R}$.
    \item $\mathcal{L}$ is a $\mathfrak{D}$-typed \textbf{data logic layer} over $\mathcal{P}$, i.e., a pair $(Q, A)$, where $Q$ is a finite set of FO($\mathfrak{D}$) queries over $\mathcal{P}$, and $A$ is a finite set of actions over $\mathcal{P}$.
    \item $\mathcal{N}$ is a $\mathfrak{D}$-typed \textbf{control layer} over $\mathcal{L}$, \ie a tuple $(P, T,F_{in},$ $F_{out}, F_{rb}, \allowbreak \texttt{color}, \allowbreak\texttt{query}, \texttt{guard}, \texttt{action})$, where:
      \begin{compactitem}[\it (i)]
      \item $P=P_c \uplus P_v$ is a finite set of places, partitioned into control places $P_c$ and view places $P_v$, %so-called
      \item $T$ is a finite set of transitions,
      \item $F_{in}$ is an input flow from $P$ to $T$,
      \item $F_{out}$ and $F_{rb}$ are respectively output and roll-back flows from $T$ to $P_c$,
      \item \texttt{color} is a color assignment over $P$ (mapping $P$ to a Cartesian product of data types),
      \item \texttt{query} is a query assignment from $P_v$ to $Q$ (mapping the results of $Q$ as tokens of $P_v$),
      \item \texttt{guard} is a transition guard assignment over $T$ (mapping each transition to a formula over its input inscriptions), and
      \item \texttt{action} is an action assignment from $T$ to $A$ (mapping some transitions to actions triggering updates over the persistence layer).
      \end{compactitem}
    \item $\tau: T \to \mathbb{Q}^{\geq 0} \times (\mathbb{Q}^{\geq 0} \cup \{\infty\})$ is a timed transition guard, mapping each transition $t \in T$ to a pair of values $\tau(t) = (v_1, v_2)$, where $v_1$ is a non-negative rational number, and $v_2$ is a non-negative rational number, or the special constant $\infty$. \qedwhite
    \end{compactitem}
\end{definition}
%

In a nutshell, the LTS of a timed db-net $\Gamma^\mathcal{B}_{s_0} = \langle S, s_0, \rightarrow \rangle$, with the (possibly infinite) set of $\mathcal{B}$-snapshots $S$, the transition relation $\rightarrow \subseteq S \times T \times S$ over states, labeled by transitions T, and both $S$ and $\rightarrow$ are defined by simultaneous induction as the smallest sets s.t.: (i) $s_0 \in S$; (ii) given a $\mathcal{B}$-snapshot $s \in S$, for every transition $t \in T$, binding $\sigma$, and $\mathcal{B}$-snapshot $s'$, if $s[t,\sigma \rangle s'$ then $s' \in S$ and $s \xrightarrow{t} s'$.
Moreover, a $\mathcal{B}$-snapshot $\langle I, m \rangle$ is a database instance $I$ and corresponding marking $m$ in the net.
A timed db-net has a special marking $(\bullet, 0.0)$, with an age of value $0.0$ appended.
%
\begin{example}
\label{ex:unconditional_fork_tdbnet}
\cref{fig:unconditional_fork_tdbnet} denotes the non-shareable multicast pattern \tikz{\node[circle,draw,red,scale=0.5] (a) at (0,0) {\textcolor{black}{N}}} in \cref{fig:sample_ipcg} with characteristics \{(MC, 1:1), (ACC, ro),.., (SH,false), (CAP,7)\} as \tdbnet. 
%
\begin{figure}[bt]
	\centering
	\includegraphics[width=\columnwidth]{images/fork_unconditional_side_effect}
	\caption{Sample multicast with side-effects as \tdbnet}
	\label{fig:unconditional_fork_tdbnet}
\end{figure}
%
To illustrate side-effects and some of the inner workings of \tdbnet, the multicast increments a stored counter in the persistence layer for each incoming message \texttt{msg}.
On arrival of a message in control place $ch_{in}$, transition $T_1$ is enabled and fires by executing action $Inc(x)$ that deletes the current count $x$ and adds a new count $x+1$ into table \texttt{Count} as well as forwards copies of the unaltered message to control places $ch_{out_1}$ and $ch_{out_2}$ (\ie read-only access: (ACC, ro)).
\qedblack    
\end{example}

We acknowledge the brevity of the introduction of \tdbnets and will shed some more light into their workings, where required.

%The execution semantics of timed db-nets builds upon the one for standard db-nets.
%The management of bindings, guards, and database updates via actions, is kept unaltered, while additional conditions on the flow of time and the temporal enablement of transitions considering delays have to be properly tackled.
%On the one hand, as customary in temporal extensions of Petri nets, we account for the flow of time by indicating that a given amount of time is passing while the net is not firing any transition.
%This results in incrementing the delay of tokens accordingly.
%On the other hand, the enablement of transitions has to be revised by checking whether the ages of tokens that the transition intends to consume match the delay window attached to the transition.

%Technically, we proceed as follows.
%We introduce a special domain $\mathbb{A}$ in $\mathfrak{D}$ capturing the age of tokens.  
%We assume that \emph{every} control place $p$ is typed with a color that contains, as a last component, $\mathbb{A}$.
%Consequently, a marking now has also to assign an age to each token.
%In addition, we also assume that all arc inscriptions carry the age of matching tokens.

%With this intuition at hand, we reconstruct the formal definition of enablement and firing given in \cite{DBLP:journals/topnoc/MontaliR17}, as follows (see in particular the last two conditions).

%\begin{definition}[Transition Enablement~\cite{DBLP:conf/edoc/0001RMRS18,ritter2019formal}] %\label{def:enablement}
%	Let $B$ be a timed db-net $\langle \mathfrak{D},\mathcal{P},\mathcal{L},\mathcal{N},\tau \rangle$, and $t$ a transition in $\mathcal{N}$ with $\tau(t) = \langle v_1,v_2\rangle$.
%	Furthermore, let $\sigma$ be a binding for $t$, i.e., a substitution $\sigma: \mathit{Vars}(t) \to \Delta_{\mathfrak{D}}$, where $\mathit{Vars}(t)= \mathit{InVars}(t) \cup \mathit{OutVars}(t)$.	
%	A transition $t \in T$ is \emph{enabled} in a $B$-snapshot $\langle I,m \rangle$ with binding $\sigma$, if:
%	%\vspace{-0.3cm}
%	\begin{compactitem}[$\bullet$]
%		\itemsep0em
%		\item For every place $p \in \mathcal{P}$, $m(p)$ provides enough tokens matching those required by inscription $w= F_{in}(\langle p,t \rangle)$, once $w$ is grounded by $\sigma$, \ie $\sigma^\oplus(w) \subseteq m(p)$; 
%		\item The instantiated guard $\texttt{guard}(t)\sigma$ evaluates to true.
%		\item $\sigma$ is injective over $\mathit{FreshVars}(t)$, thus guaranteeing that fresh variables are assigned to pairwise distinct values of $\sigma$, and for every fresh variable $v \in \mathit{FreshVars}(t)$, $\sigma(v)$ $\not\in$ $(Adom_{\texttt{type}(v)}(I)$ $\cup$ $Adom_{\texttt{type}(v)}(m))$.\footnote{$Adom_{D}(X)$ is the set of values of type $D$ explicitly contained in $X$.}	
%		\item For each age variable $y \in \mathit{OutVars}(t)$, we have that $\sigma(y)=0$ (i.e., newly produced tokens get an age of $0$).
%		\qedwhite
%	\end{compactitem}
%\end{definition}

%Thanks to the fact that ages of tokens are properly checked and updated by the transition binding when defining enablement, we have that the definition of firing for timed db-nets is \emph{identical} to that of standard db-nets.

%\begin{definition}[Transition Firing~\cite{DBLP:journals/topnoc/MontaliR17}]  %\label{def:firing}
%	Let $B$ be a timed db-net $\langle \mathfrak{D},\mathcal{P},\mathcal{L},\mathcal{N} \tau\rangle$, and $s_1= \langle I_1,m_1 \rangle, s_2= \langle I_2,m_2 \rangle$ be two $B$-snapshots.
%	Fix a transition $t$ of $\mathcal{N}$ and a binding $\sigma$ such that $t$ is enabled in $s_1$ with $\sigma$ (cf.~\cref{def:enablement}).
%	Let $I_3= apply(action_\sigma(t),I_1)$ be the database instance resulting from the application of the action attached to $t$ on database instance $I_1$ with binding $\sigma$ for the action parameters.
%		For a control place $p$, let $w_{in}(p,t)= F_{in}(\langle p,t \rangle)$, and $w_{out}(p,t)= F_{out}(\langle p,t \rangle)$ if $I_3$ is compliant with $\mathcal{P}$, or $w_{out}(p,t)= F_{rb}(\langle p,t \rangle)$ otherwise.
%		We say that $t$ \emph{fires} in $s_1$ with binding $\sigma$ producing $s_2$, written $s_1[t,\sigma \rangle s_2$, if:
%	\begin{compactitem}[$\bullet$]
%		\itemsep0em
%		\item if $I_3$ is compliant with $\mathcal{P}$, then $I_2$=$I_3$, otherwise $I_2$=$I_1$;
%		\item for each control place $p$, $m_2$ corresponds to $m_1$ with the following changes: $\sigma^{\oplus}(w_{in}(p,t))$ tokens are removed from $p$, and $\sigma^{\oplus}(w_{out}(p,t))$ are added to $p$.	 In formulae: $m_2(p_c)= (m_1(p_c)-\sigma^{\oplus}(w_{in}(p,t))) + \sigma^{\oplus}(w_{out}(p,t))$\qedwhite
%	\end{compactitem}
%\end{definition}
%

%The execution semantics of a timed db-net then follows the standard construction, modulo two refined aspects.
%First, the original (non-timed) definition of enablement in \cite{DBLP:journals/topnoc/MontaliR17} is substituted with its refined version in \cref{def:enablement}.
%Second, when constructing the transition system, we also add the (infinitely many) transitions dealing with the flow of time.
%This is done by simply imposing that every $B$-snapshot $\langle I,m \rangle$ is connected to every $B$-snapshot of the form $\langle I',m' \rangle$ where $I' = I$ (i.e., the database instances are identical) and $m'$ is identical to $m$ but for the ages of tokens, which all get increased by the same, fixed amount $x \in \mathbb{Q}$ of time.

%In the following, given two $B$-snapshots $s$ and $s'$, we write $s \rightarrow s'$ if there exists a direct transition from $s$ to $s'$ in the transition system that captures the execution semantics of $B$ starting from a given initial snapshot $s_0$.
%We also write $s \xrightarrow{*} s'$ if there is a sequence of transitions leading from $s$ to $s'$.
